Bandit optimisation of functions in the Mat\'ern kernel RKHS

We consider the problem of optimising functions in the reproducing kernel Hilbert space (RKHS) of a Mat\'ern kernel with smoothness parameter $\nu$ over the domain $[0,1]^d$ under noisy bandit feedback. Our contribution, the $\pi$-GP-UCB algorithm, is the first practical approach with guaranteed sublinear regret for all $\nu>1$ and $d \geq 1$. Empirical validation suggests better performance and drastically improved computational scalablity compared with its predecessor, Improved GP-UCB.

==> figs/alg-cover.tex <==
\begin{algorithm}[t]
\begin{algorithmic}
\small\Require{initial horizon $H_0$, dimensionality $d$, and kernel parameter $\nu$.}\\

\State Let $q={\frac{d(d+1)}{d(d+2)+2\nu}}$ and $b=\frac{d+1}{d+2\nu}$. \\ 

\Function{UpdateCover}{$\mcA$, $D$}
    \If{$\exists i\in\N \colon |D| = 2^i H_0$}
        \State $\mcA \gets \mcR([0,1]^d, (2|D|)^{-q/d})$
    \EndIf\\
    
    \While{$\{A' \in \mcA \colon |\dat{A'}{}|+1 > \radius{A'}^{-1/b} \} \neq \emptyset$}
        \State Choose any $A\in \{A' \in \mcA \colon |\dat{A'}{}|+1 > \radius{A'}^{-1/b}\}$
            \State $\mcA \gets (\mcA \setminus \{ A\}) \cup \mcR(A, 2^{-b} \radius{A})$
        
    \EndWhile
    \State\Return{$\mcA$}
\EndFunction

\end{algorithmic}
\caption{\small{$\pi$-Cover construction}}
\label{alg:pi-cover}
\end{algorithm}


==> figs/alg-ucb.tex <==
\begin{algorithm}[t]
\begin{algorithmic}
\State Initialise $\dat{\dom}{0}=\emptyset$
\For{$t=1,2,\dotsc$}
    \State Construct covering set $\mcA_t$
    \State Find an $x_t \in \argmax{x\in\dom}\UCB_t(x)$ 
    \State Update $\dat{\dom}{t} \gets \dat{\dom}{t-1} \cup     \{(x_t,y(x_t))\}$ 
\EndFor

\end{algorithmic}
\caption{$\pi$-GP-UCB}
\label{alg:pi-ucb}
\end{algorithm}

% \For{$A\in\mcA_t$ such that $|\dat{A}{t}|+1 > \radius{A}^{-1/b}$} 
    % \State $\mcA_{t} \gets (\mcA_t \setminus \{ A\}) \cup \mcR(A, 2^{-b} \radius{A})$
% \EndFor


==> figs/diagram-cover.tex <==

\tikzset{
  cross/.pic={
    \draw[pic actions] 
      (2pt,2pt) -- (-2pt,-2pt)
      (2pt,-2pt) -- (-2pt,2pt);
  },
}

\begin{tikzpicture}
% Domain
\draw [densely dotted] [|-|] (0,1) -- (6,1);
\node[] at (6.5,1) {$\dom$};

% data
\foreach \x in {1,2, 2.2, 2.3, 2.4, 2.7,3.1, 3.2, 3.3,4,4.9,4.8,4.65,4.6,4.1}
{
  \pic[line width=0.5pt] at (\x,1) {cross}; 
}


% B^0
\draw  [|-|] (0,0) -- (2,0);
\draw [dashed][-|] (2,0) -- (4,0);
\draw [dashed][-|] (4,0) -- (6,0);
\node[] at (6.5,0) {$\mcB^0_t$};

% B^1

\draw [dashed][|-|] (2,-1) -- (3,-1);
\draw [-|] (3,-1) -- (4,-1);

\draw [dashed][-|] (4,-1) -- (5,-1);
\draw [-|] (5,-1) -- (6,-1);
\node[] at (6.5,-1) {$\mcB^1_t$};


% B^2
\draw [|-|] (2,-2) -- (2.5,-2);
\draw [-|] (2.5,-2) -- (3,-2);
\draw [|-|] (4,-2) -- (4.5,-2);
\draw [-|] (4.5,-2) -- (5,-2);
\node[] at (6.5,-2) {$\mcB^2_t$};
\end{tikzpicture}

==> imports.tex <==
\RequirePackage{booktabs}
\RequirePackage[round]{natbib}
\bibliographystyle{plainnat}
%\RequirePackage{subcaption}
\RequirePackage{graphicx}
\RequirePackage{algorithm,algpseudocode}
\RequirePackage{amsmath,amsthm,amssymb,amsbsy,mathtools,thm-restate}
\RequirePackage{breqn}
\RequirePackage[noabbrev]{cleveref}
\RequirePackage{xcolor}
\RequirePackage{enumitem}
\RequirePackage{multirow}
\RequirePackage{breqn}
\RequirePackage{multirow}
\RequirePackage{tikz}
\RequirePackage{enumitem}
\RequirePackage{dblfloatfix}

%%% THEOREMS
\declaretheorem[name=Proposition]{prop}
\declaretheorem[name=Corollary,sibling=prop]{cor}
\declaretheorem[name=Theorem,sibling=prop]{theorem}
\declaretheorem[name=Lemma,sibling=prop]{lem}
\declaretheorem[name=Remark,sibling=prop]{rem}
\declaretheorem[name=Assumption]{ass}
\declaretheorem[name=Definition]{defn}


\expandafter\let\expandafter\oldproof\csname\string\proof\endcsname
\let\oldendproof\endproof
\renewenvironment{proof}[1][\proofname]{%
  \oldproof[{\bf #1}.]%
}{\oldendproof}
% \Crefname{thm}{Theorem}{Theorems}
% \Crefname{lem}{Lemma}{Lemmas}

%%% TODONOTES AND PAGE SIZE HACK TO MAKE IT VIABLE
\usepackage{marginnote} 
\let\marginpar\marginnote
\RequirePackage[textsize=small]{todonotes}
% \paperwidth=\dimexpr \paperwidth + 6cm\relax
% \oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
% \evensidemargin=\dimexpr\evensidemargin + 3cm\relax
% \marginparwidth=\dimexpr \marginparwidth + 3cm\relax
% \setlength{\marginparwidth}{4cm}

==> introduction.tex <==
% Consider citing 
% http://jmlr.org/papers/volume16/zhang15d/zhang15d.pdf

Global optimisation is the task of identifying an optimum of a given function $f\colon \dom \mapsto \R$ on its domain $\dom$, given the ability to query the function at chosen locations. The function observations may be subject to noise, such that for a query point $x_t$ selected at step $t$, the algorithm observes $y(x_t) = f(x_t) + \epsilon_t$, for $\epsilon_t$ some noise variable. For the task to be tractable, some assumptions have to be made about the domain $\dom$, regularity conditions on $f$ and on the distribution of $\epsilon_t$. For set of assumptions, the performance of a global optimisation algorithm is typically characterised by either, the suboptimality of the best prediction it can make at time $T$, or cumulative sub-optimality of each point selected for evaluation by the algorithm until time $T$, referred to as the regret. Bounding the regret by a sublinear function of $T$ is a stronger statement, as it implies a bound on the best prediction sub-optimality, while the reverse does not hold. Within this work, we focus on the latter characterisation of performance, which also coincides with bandit optimisation, for an (inifinitely armed) bandit. The bandit problem is a classic example of the exploration-exploitation trade-off, where the algorithm has to decide whether to select points close to the current estimates of the optimum, or to explore the domain. The bounds derived here may therefore be of interest beyond the setting of global optimisation.

Global optimisation algorithms can then, broadly speaking, be categorised by the types of regularity conditions assumed. Common assumptions include: finite dimensional linear functions; Lipschitz optimisation, where a known Lipschitz constant for $f$ is assumed; Bayesian optimisation, where $f$ is assumed to have been sampled from a Gaussian process with a known kernel; or the assumption that the function belongs to the RKHS associated with a known kernel. The focus of this work is on the assumption that $f$ belongs to the RKHS of a Mat\'ern family kernel with parameter $\nu>1$ \citep{stein}, the observations of $f$ available are corrupted with additive subGaussian noise, and that the domain is $[0,1]^d$. This is a hard problem: upper bounds on regret for Bayesian optimisation for a sample from a Gaussian process with a known Mat\'ern family kernel are below the lower bounds on regret for optimisation of functions in the Mat\'ern RKHS. For algorithms dealing with functions belonging to a known RKHS on a domain $\dom$ of arbitrary dimensionality $d$, existing regret bounds are only sublinear for for an RKHS belonging to a kernel with an exponentially decaying operator spectrum, as in, for example, the Squared Exponential kernel. This is equivalent to the set of infinitely differentiable functions. The RKHS corresponding to a Mat\'ern kernel with parameter $\nu$ finite, on the other hand, corresponds to an assumption that the operator spectrum follows a power law decay. The Mat\'ern kernel RKHS is in turn equivalent to a Sobolev (detail) space, and contains the RKHS of the squared exponential as a strict subset. Furthermore, the assumption that the function $f$ is in the RKHS associated with a Mat\'ern family kernel with $\nu>1$ is distinct from assumptions of a known Lipschitz constant. The only existing sublinear regret bounds for global optimisation of functions in the Mat\'ern RKHS require that that the dimensionality of the domain $d$ is low, or that the function is very smooth; specifically, that $2\nu > d(d + 1)$. 

\begin{table}[htb]
    \centering
    \caption{A comparison of regret bounds for the optimisation of functions in the RKHS of a Mat\'ern kernel. Upper bounds hold require $\nu>1$, lower bound holds for all $\nu$.}
    \label{tab:bounds}
    \begin{tabular}{c c c}
    \toprule
          \small Lower bound & \small Existing upper bound & \small Our upper bound \\
         \small \citet{scarlett17lower} & \small \citet{srinivas2010gaussian} & \small --- \\
    \midrule
         $\Omega\Big(T^{\frac{d+\nu}{d+2\nu}}\Big)$ & 
         $\mcO\Big(T^{\frac{3d(d+1) + 2\nu}{2d(d+1) + 4\nu}}\Big)$ & 
         $\mcO\Big(T^{\frac{d(2d+3) + 2\nu}{d(2d+4) + 4\nu}}\Big)$ \\
    \bottomrule
    \end{tabular}
\end{table}

Our main contribution is the Partitioned Improved Gaussian Process Upper Confidence Bound ($\pi$-GP-UCB) algorithm, an extension of the classic GP-UCB and Improved GP-UCB algorithms, which we review in \cref{sec:background}. We prove that, with arbitrarily high probability, our algorithm attains sublinear regret for functions in the Mat\'ern RKHS on the domain $[0,1]^d$, for all $\nu > 1$ and all $d\geq 1$. We summarise how it fits into the existing literature in table \cref{tab:bounds}: for the RKHS corresponding to the Mat\'ern kernels with low parameter $\nu$, i.e. functions with minimal smoothness assumptions, our bounds can be seen to compare favourably with the algorithm-agnostic lower bounds for this task. In addition, we use insights from the regret bounds for $\pi$-GP-UCB to provide stronger regret bounds for the GP-UCB algorithm in the context of Bayesian optimisation.  

